DTG : Diffusion-based Trajectory Generation for Mapless Global Navigation

We present a novel end-to-end diffusion-based trajectory generation method, DTG, for mapless global navigation in challenging outdoor scenarios with occlusions and unstructured off-road features like grass, buildings, bushes, etc. Given a distant goal, our approach computes a trajectory that satisfies the following goals: (1) minimize the travel distance to the goal; (2) maximize the traversability by choosing paths that do not lie in undesirable areas. Specifically, we present a novel Conditional RNN(CRNN) for diffusion models to efficiently generate trajectories. Furthermore, we propose an adaptive training method that ensures that the diffusion model generates more traversable trajectories. We evaluate our methods in various outdoor scenes and compare the performance with other global navigation algorithms on a Husky robot. In practice, we observe at least a 15% improvement in traveling distance and around a 7% improvement in traversability.

==> archive/v0.tex <==
\begin{abstract}
We present a diffusion-based trajectory generation method, DTG, for outdoor mapless global navigation in challenging campus scenarios with unstructured features like grass, buildings, bushes, etc. Given a faraway target, our approach aims at balancing both reducing the future traveling distance and maximizing the traversability (the portion of trajectories on pavements instead of undesirable off-road areas). 
We propose an end-to-end trajectory generator to handle the problem of generating traversable trajectories with short future traveling distance. Especially for the diffusion models, we present a novel Condtional RNN for efficient trajectory generation. We also propose an adaptive training method to push the training of diffusion model to generate more traversable trajectories. In addition, we highlight our benefits compared with other state-of-the-art global navigation algorithms on a Husky robot and demonstrate at least \textbf{$15\%$} improvement in traveling distance and $2$ points reduction of running into off-road areas.

% the cost-to-go estimation (the shortest traveling distance to the target) and the traversability (the portion of trajectories on pavements instead of undesirable off-road areas). 
% generates potential trajectories with the best heuristic (the shortest traveling distance to the target) only on pavements and avoids undesirable off-road areas. 
\end{abstract}


\section{Introduction}
\label{sec:intro}

Global navigation solves the problem of navigating robots in large-scale environments~\cite{ganesan2022global, gao2019global, ort2018autonomous}. Global navigation is widely used in various tasks, such as autonomous driving~\cite{ort2018autonomous, yurtsever2020survey}, last-mile delivery~\cite{hoffmann2018regulatory, chen2021adoption}, and search and rescue operations~\cite{davids2002urban}. However, the problem is not trivial and there are various challenges in global navigation tasks~\cite{huang2005online, giovannangeli2006robust, shah2022viking, liang2023mtg}.

\textit{Accurate and up-to-date global maps are not always available:} A common requirement across many global navigation strategies~\cite{ganesan2022global, gao2019global, psotka2023global} is the necessity for a global map to facilitate planning. However, obtaining a precise map poses significant challenges, particularly for outdoor navigation tasks in environments lacking paved roads or clear lane markings~\cite{ort2018autonomous}. SLAM methods~\cite{shan2020lio, shan2018lego, rosinol2021kimera} suffer from drifting issues and require frequent loop closures to maintain the quality of generated maps. Classical SLAM methods~\cite{shan2020lio, shan2018lego} also lack traversability information for navigation. Temporary construction zones and hazardous areas are also map-denied, which require online mapping~\cite{lajoie2020door, huang2005online} for map-based navigation approaches. These methods cannot plan an optimal and traversable global path until the best trajectory is explored by the robots after navigation or exploration of unknown areas. Therefore, mapless navigation is a critical problem for outdoor global navigation. Nevertheless, mapless outdoor navigation is not a trivial problem, and there are many challenges, 
including traversability analysis, optimality assurance, constraints satisfaction, etc.~\cite{giovannangeli2006robust, shah2022viking, lavalle2006planning}.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/place_holder.png}
    \caption{Front}
    \label{fig:front}
\end{figure}

\textit{Robots need to navigate in their traversable areas:} In complex outdoor scenarios, traversability analysis is critical to safely navigate robots to their targets because the outdoor environment contains various challenging terrains, plants, buildings, trees, etc~\cite{liang2022adaptiveon, weerakoon2023graspe, xiao2021learning, karnan2022vi, pokhrel2024cahsor, jardali2024autonomous}. Traditionally, perception and planning are separated into two tasks~\cite{canny1988complexity,manocha1992algebraic,lavalle2006planning}: first, use perception models to detect traversable areas for the current type of robot; second, apply the traversable constraints to the planner and plan a trajectory to move the robot. However, the traversable maps created by these approaches are not the most efficient representation of the environment for robots to process, because the robots only need encoded representation of the traversability information to understand the environment.
% This approach requires significant effort to extract all possible traversable areas in a human-visible manner, but such a method is computationally costly and not the most efficient way to encode the information for robots, which only need encoded information.
% the best for robots, and it is also computationally costly to build human-friendly \xuesu{what do you mean by human-friendly?} perceptions for navigation. 
To alleviate the issues, in DTG, we use an end-to-end diffusion-based trajectory generation structure to encode the traversability information to a vector as the input of trajectory-generation models. To sufficiently encode the traversability information we propose a novel training strategy for diffusion models by adaptively training the models with traversability losses.
% In this paper, we apply empirical training to an end-to-end structure for navigation. 


\textit{Global navigation has multiple objectives to achieve (distance and traversability) under various constraints:} For different global navigation tasks, there could be different optimality targets. Given a goal, robots are required to move to the goal heuristically~\cite{shah2022viking, kahn2021land}. The \textit{heuristic} is calculated from the estimated traveling distance to the goal in the traversable environment and large heuristic values mean a longer distance to travel in the future. For exploration tasks~\cite{lluvia2021active, keidar2014efficient} the optimality is to efficiently explore the current environment. For rescue or moving robots in hazardous environments, robots' safety is a higher priority~\cite{davids2002urban}. To achieve these optimalities, different constraints are also applied to the navigation problems, such as mobility constraints of the robot and traversability constraints. The navigation problem we are solving is to generate trajectories w.r.t. the optimality of traveling distance (heuristic) in complex mapless outdoor scenarios under the constraints of traversability. In this approach, we generate heuristic and traversable trajectories to navigate the robot to its faraway goal in a large-scale environment. 

Diffusion models show excellent performance in generating new trajectories~\cite{chi2023diffusion} than other approaches, such as CVAE (Conditional Variational Auto-Encoder)~\cite{cvae}, GANs (Generative Adversarial Networks)~\cite{creswell2018generative}. However, current diffusion models are used to generate trajectories close to ground truth trajectories, which have the best heuristic in traversable areas but cannot apply traversability constraints to the generated trajectories, which makes the trajectories not safe for real-world applications. In our approach, besides training generated trajectories similar to ground truth, we also applied traversability constraints to push the trajectory distributions more to traversable areas. 
% For different global navigation tasks, there could be different optimality targets. Given a goal, robots are required to move to the goal heuristically~\cite{shah2022viking, kahn2021land}. The \textbf{heuristic} is calculated from the estimated traveling distance to the goal in the traversable environment and large heuristic values mean a longer distance to travel in the future. For exploration tasks~\cite{lluvia2021active, keidar2014efficient} the optimality is to efficiently explore the current environment. For rescue or moving robots in hazardous environments, robots' safety is a higher priority~\cite{davids2002urban}. The navigation problem we are solving is to generate trajectories w.r.t. the optimality of traveling distance (heuristic) in complex mapless outdoor scenarios under the constraints of traversability. In this approach, we generate heuristic and traversable trajectories to navigate the robot to its faraway goal in a large-scale environment.

% \textbf{Trajectories should be generated under different constraints:} Given the traversability and also the goal for navigation, we need to generate trajectories to satisfy mobility constraints and to achieve the optimality on different dimensions, such as less traveling distance or running time staying on preferred terrain. Traditional approaches, such as model predictive control~\cite{kouvaritakis2016model, xiao2022learning} or Velocity-Obstacle-based algorithms~\cite{liang2021vo, gopalakrishnan2017prvo}, require numerous assumptions of the environment and robot's motions. Sequential neural networks~\cite{altche2017lstm, varadarajan2022multipath} demonstrated good performance in trajectory prediction, but they highly rely on historic trajectories. To generate trajectories with the robot's observations, generative models show good performance in trajectory generation tasks~\cite{gupta2018social, liang2023mtg, chi2023diffusion}. In this project, we use generative models to perform trajectory generation. Among different generative models, such as CVAE (Conditional Variational Auto-Encoder)~\cite{cvae}, GANs (Generative Adversarial Networks)~\cite{creswell2018generative}, Diffusion models~\cite{ho2020denoising}. Diffusion models show excellent performance in generating new trajectories~\cite{chi2023diffusion} than other approaches. However, current diffusion models are used to generate trajectories close to ground truth trajectories, which have the best heuristic in traversable areas but cannot apply traversability constraints to the generated trajectories, which makes the trajectories not safe for real-world applications. In our approach, besides training generated trajectories similar to ground truth, we also applied traversability constraints to push the trajectory distributions more to traversable areas. 

\textbf{Main results: } We present a novel approach, DTG, to generate trajectories for global navigation in complex outdoor mapless environments. Based on Diffusion generators, we propose an end-to-end trajectory generator to generate heuristic and traversable trajectories to the robot's targets. The generated trajectories are also evaluated by the confidence of their traversability for navigation. We also demonstrate the benefits of our approach, DTG, in complex outdoor scenarios including bushes, grass, and other off-road non-traversable areas. DTG achieves at least $15\%$ improvement in traveling distance and $2$ points increase in traversability of generated trajectories. The major contributions include:
\begin{enumerate}
    \item \textbf{Diffusion-based Trajectory Generator with Traversability Training Strategy: }  We propose a novel diffusion-based trajectory-generation structure to generate heuristic trajectories in traversable areas for global navigation tasks. Specifically, we propose a conditional RNN structure to efficiently denoise the trajectories. 
    
    \item \textbf{Adaptive Training Traversability:} Besides the structure, we propose a new method to adaptively add traversability loss to train the trajectory generation to generate trajectories only on traversable areas.
    % \item \textbf{Using Bayesian-based traversability estimation to improve the safety of generated trajectories: } We use cross-attention~\cite{vaswani2017attention} to process the relationship between the generated trajectories and the robot's current observation. We apply CVAE~\cite{cvae} on the traversability estimation to provide both the traversability value and its confidence. 
    \item \textbf{Performance improvement in global navigation:} We compared with the state-of-the-art trajectory generation approaches (ViNT~\cite{shah2023vint}, NoMaD~\cite{sridhar2023nomad} and MTG~\cite{liang2023mtg}) for outdoor global navigation with at least {$\mathbf{15\%}$} improvement in heuristic and \textbf{2} points improvement in traversability.
    We also compared the trajectories' traversability in complex outdoor scenarios with various off-road terrains, such as grass, buildings, and trees. Around corners our model generates trajectories with better traversability w.r.t. the geometric shape of the traversable areas, and DTG can also generate trajectories with higher heuristics in narrow spaces. Our proposed CRNN also achieves comparable traversability and heuristic compared with UNet, but our model is much faster and smaller.
\end{enumerate}



\section{Prior Work and Background}
\label{sec:background}
In this section, we review the related works of trajectory generation in challenging outdoor navigation.

% outdoor navigation
\textbf{Outdoor Navigation: } Moving robots in an outdoor environment has many challenges, for example, different complex terrains~\cite{weerakoon2023graspe, xiao2021learning, karnan2022vi, pokhrel2024cahsor, datar2023toward,canny1988complexity,manocha1992algebraic} with grass, bushes, mud, sharp elevation changes, etc. Outdoor motion planning approaches handle the problem of stably and safely moving robots on different terrains~\cite{liang2022adaptiveon, weerakoon2023graspe}, while reinforcement learning~\cite{xu2023benchmarking, xu2021applr, xu2021machine} approaches are used to train the policy neural network to generate waypoints or actions to move the robot. For global planning, given a far target, traditionally a global map is required to generate a path to guide local planning~\cite{fusic2021optimal, li2021openstreetmap}. Therefore, accurate localization methods~\cite{akai2017robust, lowry2015visual} are also required to provide the real-time pose of the robot to follow the path. Thus, classical map-based global navigation approaches are computationally intensive and also require a significant amount of effort to maintain the maps. However, maintaining an accurate map is not easy in some satellite-denied or hazardous areas~\cite{zhai2020coal}. Shah et al.~\cite{shah2023vint}, Sridhar et al.~\cite{sridhar2023nomad}, and Hirose et al.~\cite{hirose2023exaug} handle the problem by generating a topological map and extract images as subgoals for outdoor navigation. By comparing the similarities between the current observation and the saved images, the models are trained to generate trajectories to the most similar subgoal. However, those approaches do not completely solve the problem of requiring a map, since they still need to run robots in the environment to collect the subgoal images before navigation. Mapless navigation is the task of navigating robots without a map. Giovannangeli et al.\cite{giovannangeli2006robust} and AdaptiveON~\cite{liang2022adaptiveon} generate actions in a mapless manner, but they are for motion planning and do not handle long-distance navigation. MTG~\cite{liang2023mtg} provides trajectories for long-distance navigation but only generates trajectories to cover traversable areas instead of choosing the best trajectory to navigate the robot. In our approach, given a faraway target in large-scale outdoor environments without a map, DTG generates a traversable trajectory with the best heuristic to the target and we also provide a traversability estimation to better choose a consistently traversable trajectory during navigation.



% traversability analysis
\textbf{Traversability Analysis: } Traversability analysis is often implied by the approaches separating perception and planning~\cite{fan2021step, gasparino2022wayfast, jonasfast, sikand2022visual}, where multiple sorts of sensors are used to observe the scenarios and extract the traversable areas for certain types of robots~\cite{suger2015traversability, xue2023traversability}. RGB or RGB-D cameras are widely used for terrain analysis, for example, Hosseinpoor et al.~\cite{hosseinpoor2021traversability} and Frey et al.~\cite{jonasfast} use cameras to segment the terrains and generate a cost map for navigation. Lidar is another widely used sensor for traversability estimation~\cite{xue2023traversability, Fankhauser2018ProbabilisticTerrainMapping}, where geometric information is extracted from the observation to build an elevation map. However, those methods highly rely on the cost/elevation maps for navigation, and those maps are friendly for human visualizations but computationally costly for robots to process the perception information because robots can directly process encoded information of the environment. To solve this problem, end-to-end learning methods~\cite{xiao2022motion} help to implicitly encode useful information in the networks for navigation~\cite{liang2022adaptiveon, liang2023mtg}. By training with certain rewards or losses, their neural networks encode useful information for certain navigation tasks. In this project, we also use an end-to-end learning approach to encode the observation information.


% trajectory generation
\textbf{Trajectory Generation: } Many trajectory generation methods for outdoor scenarios are for autonomous driving~\cite{varadarajan2022multipath, nayakanti2023wayformer, shi2022motion}, which predicts the future waypoints of the car based on the historic positions. There is also trajectory generation for small robots~\cite{kahn2021land, shah2022viking, shah2023vint}. Those approaches take subgoal images and current images to estimate the similarity between them and generate trajectories with a low traversability cost to the subgoal. However, these methods highly depend on the distance of the subgoal images and require the images to be very close. If the subgoal images are very different from the current observations, the model gets confused, so sophisticated subgoal choices are necessary~\cite{shah2023vint}. In addition, these approaches require the subgoals to be sequential to the final goal, and the robot has to travel from the starting position to the goal without deviation, so these methods are not completely mapless approaches.
MTG~\cite{liang2023mtg} generates trajectories in traversable areas and also continuous space, but it doesn't consider trajectory optimally in terms of distance to the goals. 
% People doing manipulations generate trajectories using different methods~\cite{chi2023diffusion, hauser2010fast}, but the manipulation task is very different from the navigation tasks, manipulation tasks have a third-person view of the scenario and the robot, but for navigation, we only have robot's first-person view to the environment. 
In our approach, we propose a novel diffusion-based mapless trajectory generator and also trained by generating trajectories only in traversable areas.

% generative models
\textbf{Generative Models: } Sequential networks have been widely used in trajectory prediction tasks. Researchers use sequential networks, e.g., LSTM~\cite{altche2017lstm} and Gaussian Mixture Models~\cite{varadarajan2022multipath} to predict trajectories, but those trajectory-prediction approaches heavily rely on the historic trajectories of the robot. Bayesian-based approaches are also applied to the trajectory generation problem~\cite{liang2023mtg, yang2020online}, and those approaches also calculate the (un)certainties of the generated trajectories. Later GANs (Generative Adversarial Networks) demonstrated good performance in trajectory prediction tasks~\cite{gupta2018social}.
With the development of generative models, Diffusion models~\cite{ho2020denoising, song2020denoising} start to play an increasingly important role in robotics~\cite{chi2023diffusion, shah2023vint} and they demonstrated better performance compared with NoMad~\cite{sridhar2023nomad}, MTG~\cite{liang2023mtg}, and CVAE-based generator~\cite{cvae}. In this paper, we also use diffusion models to generate trajectories in traversable areas.

\section{Approach}
\label{sec:approach}

In this section, we define our problem and describe how DTG addresses such a problem. 


\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/architecture.png}
\caption{\textbf{DTG Architecture:} DTG has three models: \textbf{Perception Encoder}, \textbf{Diffusion Model} and \textbf{Traversability Estimator}. Perception Encoder encodes the perception information to a vector. The diffusion Model takes a Gaussian distribution to a trajectory $\hat{\btau}$ under the condition of the perception information. The Traversability Estimator takes the generated trajectory and the perception information to estimate the traversability $\hat{v}_t$ of the trajectory and also provides the confidence of the traversability.}
    \label{fig:architecture}
\end{figure*}

\subsection{Problem Definition}
\label{sec:problem_definition}
The problem we are solving is outdoor mapless global navigation. Given a very distant goal $g\in\co_g$, which is assumed to be mostly out of the vision of the robot in a large-scale environment, our model generates trajectories in the robot's traversable areas with the best heuristic (estimated distance) to the target. We have a similar assumption as MTG~\cite{liang2023mtg} that the trajectory generator ignores small and dynamic obstacles, which can be avoided by local planners.

The perceptive sensors in our approach include a 3D Lidar and an odometer of the robot. As CrowdSteer~\cite{liang2021crowd} and MTG~\cite{liang2023mtg}, we also use three consecutive frames of Lidar perception, $\co_l$, to capture the environment in the robot's vicinity. The odometer provides the latest ten consecutive frames of velocities of the robot, $\co_v$. The goal, $g\in \co_g$, in this global navigation task is at least $40$ meters from the robot. Thus, the observation contains $\co = \set{\co_l, \co_v, \co_g}$. Given the observation $\co$, our trajectory generator $m_\theta$ generates a traversable and heuristic trajectory $\btau=\set{w_1,..., w_M}$ to the target, where $M=16$ is the number of waypoints and $w_m = \set{x_m, y_m}$. The generated trajectory has a length of 15 meters, $\abs{\btau} = 15m$, starting from the robot. We define the heuristic of the trajectory $\btau$ as the length of the shortest path from the last waypoint $\tau_l$ of $\btau$ to the target $g$. For each observation $o\in \co$, we have $m_\theta(o) = \btau$ and $m_\theta(o)_l = \tau_l$. 

\begin{align}
    \hat{\theta} = \argmin{\theta} \left( h(m_\theta(o)_l, g) + \beta f(m_\theta(o), \Tilde{\ca}) \right)
\end{align}
where $h(\cdot,\cdot)$ represents the heuristic function between the last waypoint $\tau_l$ and goal $g$. $\ca$ is the traversable area around the robot and $\Tilde{\ca}$ represents non-traversable areas. $\beta$ is a hyperparameter and $f(\cdot, \cdot)$ calculates the traversability of trajectory $\btau$, which is the portion of non-traversable areas covered by the trajectory $\btau$. Therefore, the inference of our approach only takes $o\in \co$ as input, but to train the models, we require $\ca$ to calculate the traversability ground truth.

Similar to MTG~\cite{liang2023mtg}, DTG builds a traversability map for training. The heuristic function $h(\cdot,\cdot)$ can be handled by the A* algorithm, starting from the last waypoint $\tau_l$ to the goal $g$, and the heuristic is the length of the calculated A* path. The non-traversable area $\Tilde{\ca}$ can also be directly extracted from the traversability map. Then, the problem becomes optimizing the heuristics and traversability of the generated trajectory.  

Since we already have the traversability map and use path planning methods to calculate heuristics of trajectories, we can directly calculate the most heuristic and also traversable trajectory as the ground truth of the generated trajectory in the training. 
% If we can train the model to generate the same trajectory, the heuristic would be the best. 
Thus, we redefine the problem as 

\begin{align}
    \hat{\theta} = \argmin{\theta} \left( d(m_\theta(o), \btau_{gt})  + f(m_\theta(o), \Tilde{\ca}) \right)
    \label{eq:problem_definition}
\end{align}
where $\btau_{gt}$ is the ground truth of the most heuristic trajectory given the goal $g$, and $d(\cdot,\cdot)$ calculates the distance between the generated trajectory and the ground truth trajectory $\btau_{gt}$. Thus, this problem can be solved by a supervised learning strategy.

\subsection{Architecture}
Figure~\ref{fig:architecture} shows the architecture of our approach, DTG. There are three models in the pipeline: \textbf{Perception Encoder} $P_\theta(\cdot)$, \textbf{Diffusion Model} $D_\theta(\cdot)$, and \textbf{Traversability Estimator} $E_\theta(\cdot)$. 
Here we abuse the notation and denote all model parameters as $\theta$. The detail of the layer configurations is in the Appendix~\ref{appdenix}.

\subsubsection{\textbf{Perception Encoder}}
\label{sec:perception}
The Perception Encoder encodes the Lidar, Velocities, and Target information into a vector as the input of the Diffusion Model:
\begin{align}
    \e_o = P_{\theta}(o_l, o_v, g) = p^e_{\theta}(p^c_{\theta}(o_l), p^v_{\theta}(o_v), g)
\end{align}
where $o_l\in\co_l$, $o_v\in\co_v$ and $g\in\co_g$. $p^c_\theta(\cdot)$ represents the model PointCNN~\cite{hua2018pointwise} with the a 0.08m voxelization radius, $p^v_\theta(\cdot)$ and $p^e_\theta(\cdot)$ are all sequences of Linear layers. As shown in Fig.~\ref{fig:architecture}, $p^c_{\theta}(o_l), p^v_{\theta}(o_v)$ and $g$ are concatenated together to the last perception layer $p^e_\theta(\cdot)$. The output of the Perception Encoder is a vector, $\e_o$.

\subsubsection{\textbf{Diffusion Model}}
\label{sec:diffusion}
The diffusion model processes the observation information $\e_o$ and generate trajectory $\hat{\btau}$. In recent years multiple diffusion training strategies have been proposed, such as DDPM~\cite{ho2020denoising}, DDIM~\cite{song2020denoising}, and VDM~\cite{vdm}. Training networks to predict proper noise or to predict trajectory are mathematically equivalent, and in our approach, we predict trajectory by the diffusion model. In this section, we only explain the models predicting trajectories with the VDM~\cite{vdm} strategy. Our diffusion generator contains N steps and in each step, the noise is added and the noisy trajectory is $\Tilde{\x}_t = \sqrt{\alpha_t} \x_{t-1} + \sqrt{1-\alpha_t} \epsilon$, where $\alpha_t$ is the noising ratio in step $t \in \set{1,..., N}$ and $\epsilon$ is the noise. The predicted trajectory in step $t$ is $\hat{\x}_{t-1}=R_\theta(\Tilde{\x}_t, t)$, where $R_\theta(\cdot)$ is an RNN cell in Figure~\ref{fig:architecture}. Because we also require generated trajectories to be all in traversable areas, we need the generator to also have environmental information. Inspired by~\cite{chi2023diffusion}, we propose a conditional RNN to take the environment information and step $t$ as conditions of the generator, $R_\theta(\Tilde{\x}_t, t, \c)$, where $\c = d^e(\e_0) $ is the encoded environment information and $d^e(\cdot)$ is the encoder of the observation information, as shown in \ref{fig:architecture}. Thus, we have the RNN cell:
\begin{align}
d^h_\theta(t,\c) &=f^2_\theta(f^1_\theta(d^p(t)),\c)=\h\\
    r^k_\theta(\Tilde{\x}_t, \h) &= d^g_\theta(\Tilde{\x}_t, \h) \\
    R_\theta(\Tilde{\x}_t, t,\c) &= r^1_\theta( \Tilde{\x}_t, ... r^1_\theta(\Tilde{\x}_t, \h))
\end{align}
where $d^h(\cdot)$ calculates the hidden vector $\h$ for GRU cells. $d^p(\cdot)$ represents Sinusoidal positional embedding. $f^1_\theta(\cdot)$ and $f^2_\theta(\cdot)$ are all Linear layers. $k\in \set{1,..., K}$ represents the steps in the RNN model, and each step is $r^k_\theta(\cdot)$. $d^g_\theta(\cdot)$ is GRU cell and $\h$ is the hidden vector for the GRU cell. We also compared with U-Net~\cite{chi2023diffusion} as the conditional encoder and show the results in Table~\ref{tab:ros_quanti} and demonstrate that we have comparable results and significantly less computational cost.

Given all the information above, we have the sampled trajectory:
\begin{align}
    \hat{\tau} = R_\theta(...R_\theta(\bxi, N, \c), 1, \c)
\end{align}
where $\bxi$ is sampled from a random Gaussian distribution. As shown in Figure~\ref{fig:architecture}, all RNN models share the same parameters. The output of the diffusion model composes a sequence of $\set{\Delta x_m, \Delta y_m}$, and the waypoint positions $w_m = \set{x_m, y_m}\in \hat{\tau}$ are calculated by accumulating the incremental distances.

% \subsubsection{\textbf{Traversability Estimator}}
% After trajectory generation, we can run the robot to follow the trajectory. However, because the traversability map in MTG~\cite{liang2023mtg} is not accurate enough, we want to know how confident the generated trajectories are in traversable areas, then we can update the trajectory with the highest confidence for navigation. Since our model needs to run on a small laptop in real-world experiments, we need to design a simple structure with a small computational cost for the estimation. 

% As Figure~\ref{fig:architecture}, we propose a novel Traversability Estimator based on CVAE~\cite{cvae} algorithm. Given the generated trajectory $\hat{\btau} = \set{w_1,...,w_M}$, where $w_m, m\in \set{1,...,M}$ represents the waypoints in the trajectory. The problem is formulated as maximizing the likelihood of the traversability values.
% \begin{align}
%     p(v_t|\u) &\approx \frac{1}{S}\sum_{s=1}^S p(v_t|\z^{(s)},\u), \z^{(s)} \sim \cn(\mu, \nu)
% \end{align}
% where $p(v_t|\u)$ is the probability of the traversability value $v_t$, under some condition of  vector $\u$. The probability of $v_t$ can be calculated as the expectation of the probabilities of sample $s$, where $\z$ is sampled from the distribution $\cn(\mu,\nu)$. 

% Define $p_\theta(\btau, \c, \epsilon) = \set{\z, \u}$ as the encoder of the Trajectory Estimator, where $\btau$ and $\c$ are generated trajectory and encoded environment information from the Diffusion Model and $\epsilon$ is noise sampled from Gaussian distribution $\cn(0,\I)$. Decoder $q_\theta(\z, \u)=\hat{v}_t$ estimates the traversability, we have:

% \begin{align}
%     p_\theta(\btau, \c) &= e^o_\theta(e^c_\theta(e^p(\btau), f^4_\theta(\c)), \epsilon)\\
%     q_\theta(\z, \u) &= f^5_\theta(\z, \u)
% \end{align}
% where the $\epsilon\sim\cn(0, \I)$. $f^4_\theta$ and $f^5_\theta$ are linear layers. $e^p(\cdot)$ represents the 2D sinusoidal embedding of the waypoints $w_m = \set{x_m, y_m} \in \btau$. $e^c_\theta$ is a cross-attention mechanism and we put the embedded trajectory information as query and environment information as key and value. Therefore, this process enhances the embedded trajectory information by the environment information $\c$. The function $e^o_\theta$ applies the reparameterization trick~\cite{cvae} and estimates $\mu$ and $\nu$ of the distribution, then it samples $\z$ from the estimated distribution, where $\epsilon$ introduces Gaussian noise to form the distribution as~\cite{cvae} shown in Figure \ref{fig:architecture}.


\subsection{Training Strategy}
According to the problem defined in Section~\ref{sec:problem_definition}, we have two targets to achieve: 1. reduce the distance between generated trajectories and 2. train the trajectories on traversable areas. 

\subsubsection{\textbf{Adaptive Training of Diffusion Models}}
As mentioned in Section~\ref{sec:diffusion}, our approach uses the training of predicting trajectories. According to the diffusion loss in~\cite{vdm}, we formulate our diffusion loss as
\begin{align}
    \cl_d^r = \expect{t,\epsilon_d} \left( (\text{SNR}(t-1) - \text{SNR}(t)) \norm{\hat{\x}_t - \btau_{gt}}^2_2 \right),
\end{align}
where $t\in\set{1,...,N}$ and $\epsilon_d \in \cn(0, \I)$. SNR$(t) = \frac{\Bar{\alpha}_t}{1- \Bar{\alpha}_t}$. $\Bar{\alpha}_t=\prod_{i=1}^t \alpha_i$ is defined the same as \cite{ho2020denoising}. To simplify the loss function, because SNR(t) is monotonically decreasing, $(\text{SNR}(t-1) - \text{SNR}(t))$ is always positive, and we find similar training results after removing this term. Thus, the loss function is simplified as:
\begin{align}
    \cl_d^r = \expect{t,\epsilon_d} \norm{\hat{\x}_t - \btau_{gt}}^2_2
\end{align}

The current loss function only trains the diffusion model to imitate the ground truth trajectories, and we still need to add constraints to train the generated trajectories only in traversable areas. However, because the diffusion model denoises the Gaussian distribution step by step, we cannot directly add the traversability constraint in each step or the training gets sabotaged. Thus, we propose an adaptive strategy to add the traversability constraints.

\begin{align}
    l_d^t(\btau, \Tilde{\ca}) &= \exp{\left(1 - \frac{1}{M}\sum_{m=1}^M\min{d(\Tilde{\ca}, w_m)}\right)} \\
    \cl_d^t &= \expect{t\in h( N_t, l_d(i-1)),\epsilon_d\in\cn(0,\I)} l_d^t(\hat{\x}_t, \Tilde{\ca})
    \label{eq:traversability_loss}
\end{align}
where $d(\cdot)$ calculates the distance between the current waypoint $w_m$ and its nearest non-traversable area, and the distance function clips the value to $[0-1]$ meters. We sample t from the range $h( N_t, l_d(i-1))$,  where $h(\cdot)$ is the schedule function to calculate the range of the step t. $i$ is the index of training epochs and $N_t=10$ is the maximum step number in the range. $l_d(i-1)$ saves $N_t$ values that are diffusion losses of the $N_t$ steps in the last epoch. We start from 0, if the first value of $l_d(i-1)$ exceeds threshold $H_d$, we add 1 in the range $\set{0, 1}$, and similar to the later indices, we increase the range incrementally by adding the indices when their corresponding losses get smaller than the threshold $H_d$. Finally, we have the loss function for the Diffusion Model:
\begin{align}
    \cl_d = \beta_1 \cl_d^r + \beta_2 \cl_d^t
\end{align}

% \subsubsection{\textbf{Training of Traversability Estimator}}
% The loss function to the Traversability Estimator is in the CVAE~\cite{cvae} loss format:
% \begin{align}
%     \cl_t = -\cd_{KL} (p_\theta (\hat{\btau},\c) \parallel p (\z)) + \beta_3\abs{\hat{v_t} - v_t}
% \end{align}
% where $p(\z)$ represents the prior distribution, which is $\cn(0, \I)$. $\beta_3$ is a hyperparameter. $v_t$ and $\hat{v}_t$ are the ground truth and estimated traversability, respectively.

Thus, we have the totoal loss $\cl = \cl_d + \beta_4 \cl_t$, where $\beta_4$ is a hyperparameter.



\section{EXPERIMENTS}
\label{sec:experiments}

In this section, we talk about the details of the implementation, comparisons, and ablation studies of this approach. The real-world experiment is achieved by combining the lower-level motion planner DWA~\cite{fox1997dynamic}. The details of the real-world experiment and the results are in the Appendix~\ref{appdenix}.

\subsection{Implementation}
As described in Section~\ref{sec:approach}, our major perceptive sensor is a 3D Velodyne Lidar (VLP-16), which has 16 channels and a 3Hz frequency. In this project, we choose consecutive 3 frames as the input of Lidar information. The goal is set by converting the GPS value to meters. For training the goals are randomly selected within the 60 meters and for testing, the goals are randomly selected beyond 50 meters. The training data is the same as MTG~\cite{liang2023mtg}, which is collected by the Husky robot, so the velocities are from the odometer of the Husky robot, which has a frequency of 10Hz. To keep all the perceptive information in the same time period, we select consecutive 10 frames of velocities as input. Considering the dataset in MTG~\cite{liang2023mtg} has a traversability map, we calculate the ground truth trajectory of each position by calculating the shortest path to the goal and choose the segment with a 15-meter traveling distance from the current position and each ground truth trajectory has 16 waypoints. The training and evaluation are processed in the computer with NVIDIA RTX A5000 GPU and an Intel Xeon(R) W-2255 CPU, and the real-world experiment is executed in the lap with an Intel i7 CPU and one Nvidia GTX 1080 GPU. In the real-world experiment, the diffusion model generates trajectories in 5Hz and the traversability estimator estimates the traversability of the trajectories and keeps selecting the best trajectory during navigation.

\subsection{Evaluation}

In this section, we qualitatively and quantitatively evaluate DTG compared with different state-of-the-art methods. We also show the ablation study of each component of the design.

\textbf{Traversability: } Given a trajectory $\hat{\tau}$, the traversability is calculated as Equation \ref{eq:traversability}, similar as the traversability loss in Equation~\ref{eq:traversability_loss}. Considering the robot has a radius of 0.5 meters, we clip the distance function to $[0-0.5]$ meters:
\begin{align}
    tr = \frac{1}{M}\sum_{m=1}^M\min{d(\Tilde{\ca}, w_m)}, \;\; w_m \in \hat{\tau}
    \label{eq:traversability}
\end{align}

\textbf{Heuristic Ratio: } The heuristic of a position in our problem is defined as the shortest traveling distance between the position and the goal. The Heuristic Ratio is to measure the ratio of the heuristic of the generated trajectory w.r.t the original heuristic. Therefore, given the trajectory length $\abs{\hat{\tau}}$, heuristic of the current position $h_c$ and the heuristic value of the last waypoint $h_t$, the heuristic ratio is defined as:
\begin{align}
    hr = 1 - \frac{\abs{h_t - h_c}}{2\abs{\hat{\tau}}}
\end{align}

\textbf{Comparisons: } As Table~\ref{tab:ros_quanti}, to evaluate the performance of our approach, DTG, we compare it with ViNT~\cite{shah2023vint}, NoMaD~\cite{sridhar2023nomad} and MTG~\cite{liang2023mtg}. In the evaluation, the traversability estimator is not applied, so the results of DTG are directly from the generative model. Because the NoMaD and ViNT requires the robot to move in the environment, we provide the sequence of images from the start to the goal, and each consecutive pair of images has a distance of around 1 meter. For MTG, we use the method to choose the best trajectory, the same as the experiment in MTG~\cite{liang2023mtg}. From Table~\ref{tab:ros_quanti}, we can see our approach outperforms others by at least $15\%$ in heuristic and 2 points in traversability. NoMaD and ViNT only take RGB images, so the robot is not very robust in generating trajectories only in traversable areas. NoMaD is slightly better than ViNT w.r.t. traversability and inference time. The MTG has relatively good traversability, but cannot choose the trajectory with the best heuristic, because in MTG the trajectories are generated by only comparing the straight distance to the goal instead of estimating the heuristic (traveling distance to the goal) of the trajectory. DTG also outperforms NoMaD and ViNT in inference time by 0.11s and 0.56s, but the model size is more than ViNT, NoMaD and MTG. As shown in Figure~\ref{fig:qualitative_results} the top row shows the generated trajectory in the camera and the bottom row shows the trajectory in the traversability map, where Cyan color represents the generated trajectory and yellow dots are the most heuristic trajectory to the goal. From the figures, we can see NoMaD generates shorter trajectories than MTG or DTG. From the Traversability Analysis column, for the turning cases, DTG can generate the trajectory aligned with the geometric shape of the traversable areas, but MTG and NoMaD do not perform well in corner situations. From the Heuristic Analysis column, even though the passage is narrower than the main road, to achieve a better heuristic DTG can still generate a trajectory to the target. 

\textbf{Ablation Study: } To evaluate the capability of different components, we also compared with DTG without traversability loss, changing our Conditional RNN to regular UNet model and we also changed the generative model from the diffusion model to CVAE~\cite{cvae}. From Table \ref{tab:ros_quanti}, our DTG has the best heuristic compared with other ablation studies. The UNet is much larger than our proposed CRNN with more than 989.51Mb and is also much slower than all other approaches, but because the UNet model is larger than CRNN, it can encode information better and generates trajectories with better traversability. Our novel model CRNN is faster and smaller than UNet but we also achieve comparable Heuristic and Traversability in trajectory generation. The DTG/t shows the model without training traversability loss, and obviously, it has the worst traversability, which is also the same situation for NoMaD. The CVAE model is smaller, but the generative capability is not as good as diffusion models. Its heuristic and traversability of the generated trajectories are worse than DTG.

To visualize the mechanism of the diffusion model in DTG, we show the output of the diffusion models, $\set{\Delta x_m, \Delta y_m}$, in Figure \ref{fig:diffusion_steps}. In Step 0, the increment distances are very random, but after several steps, the increment distances become more concentrated and also form into proper shapes.

To evaluate the performance of the Traversability Estimator, we show the confidence and also the trajectories in Figure \ref{fig:estimation}

\begin{table}[]
    \centering
    \begin{tabular}{c c c c c}
       \hline
        \multirow{2}{*}{Evaluation} & Heuristic   & Traversability & Inference & Model\\
         & Ratio ($\%$) & ($\%$)  &  Time (s) & Size (Mb) \\
       \hline
       ViNT         & 66.02 & 83.14 & 0.69  & 113.49 \\ %\hline
       NoMaD        & 64.54 & 89.93 & 0.24  & 72.67 \\ %\hline
       MTG          & 80.78 & 90.75 & 0.01  & 101.61 \\ \hline %\hline
       CVAE         & 92.26 & 90.79 & 0.01  & 113.96 \\ %\hline
       DTG/t        & 93.12 & 89.98 & 0.13  & 128.38 \\ %\hline
       DTG$_{UNet}$ & 92.94 & 92.38 & 2.09  & 1117.89 \\ %\hline
       DTG$_{CRNN}$  & 93.61 & 91.47 & 0.13  & 128.38 \\ \hline
    \end{tabular}
    \caption{\textbf{Quantitative Results:} Our approach achieves $15\%$ in heuristic and 2 points in traversability than NoMaD and MTG. Our proposed CRNN achieves comparable traversability and heuristic compared with UNet, but our model is much faster and smaller.}
    \label{tab:ros_quanti}
\end{table}


\input{qualitative}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/diffusion_steps.png}
    \caption{Diffusion Steps: In each generated trajectory, there are $16$ waypoints. This figure shows the output values of the diffusion model, those values are distance increments in each waypoint (not waypoint positions). In the beginning steps, the output contains lots of noise, and in later steps, the diffusion model denoises the increments and those values are in a more concentrated area and reasonable shape.}
    \label{fig:diffusion_steps}
\end{figure}


\section{Conclusion, Limitations and Future Work}
\label{sec:conclusion}
We present a novel diffusion-based trajectory generator for global navigation tasks. 
